Approximating submodular $k$-partition via principal partition sequence

In submodular $k$-partition, the input is a non-negative submodular function $f$ defined over a finite ground set $V$ (given by an evaluation oracle) along with a positive integer $k$ and the goal is to find a partition of the ground set $V$ into $k$ non-empty parts $V_1, V_2, ..., V_k$ in order to minimize $\sum_{i=1}^k f(V_i)$. Narayanan, Roy, and Patkar (Journal of Algorithms, 1996) designed an algorithm for submodular $k$-partition based on the principal partition sequence and showed that the approximation factor of their algorithm is $2$ for the special case of graph cut functions (subsequently rediscovered by Ravi and Sinha (Journal of Operational Research, 2008)). In this work, we study the approximation factor of their algorithm for three subfamilies of submodular functions -- monotone, symmetric, and posimodular, and show the following results: 1. The approximation factor of their algorithm for monotone submodular $k$-partition is $4/3$. This result improves on the $2$-factor achievable via other algorithms. Moreover, our upper bound of $4/3$ matches the recently shown lower bound under polynomial number of function evaluation queries (Santiago, IWOCA 2021). Our upper bound of $4/3$ is also the first improvement beyond $2$ for a certain graph partitioning problem that is a special case of monotone submodular $k$-partition. 2. The approximation factor of their algorithm for symmetric submodular $k$-partition is $2$. This result generalizes their approximation factor analysis beyond graph cut functions. 3. The approximation factor of their algorithm for posimodular submodular $k$-partition is $2$. We also construct an example to show that the approximation factor of their algorithm for arbitrary submodular functions is $\Omega(n/k)$.

==> intro-1.tex <==
\section{Introduction}\label{sec:intro}
A set function $f:2^V\rightarrow \R$ is submodular if $f(A)+f(B)\ge f(A\cap B) + f(A\cup B)$ for every $A, B\subseteq V$. 
We consider the \emph{submodular $k$-partition} problem defined as follows: The input consists of a non-negative submodular function $f:2^V\to\R_{\geq 0}$ on a finite ground set $V$ via an evaluation oracle and an integer $k\geq 2$. The goal is to find a partition $V_1,\ldots,V_k$ of $V$ into $k$ non-empty parts in order to minimize $\sum_{i=1}^k f(V_i)$. Namely, the goal is to compute
\[\min\left\{\sum_{i\in[k]}f(V_i):\{V_1,\ldots, V_k\}\text{ is a partition of }V,\ V_i\neq\emptyset\;\forall i\in[k]\right\}.\]
Throughout, we will assume that the submodular function is non-negative and denote the size of the ground set $V$ by $n$. 
We emphasize that our focus is on submodular $k$-partitioning when $k$ is part of input 
%The focus of this work is on submodular $k$-partitioning problem where $k$ is part of input 
(see \cite{CC22-j} for a discussion of the problem for fixed constant $k$).
%We refer the reader to \cite{CC22-j} for a discussion on the status of submodular $k$-partition problem for fixed constant $k$.  
For arbitrary submodular functions, the problem is NP-hard \cite{GH94}, does not admit a $(2-\epsilon)$-approximation assuming polynomial number of function evaluation queries \cite{San21}, does not admit a $n^{1/(\log\log n)^c}$-approximation for every constant $c$ assuming the Exponential Time Hypothesis \cite{CL20}, and 
the best approximation factor that is known is $O(k)$ \cite{ZNI05, OFN12}. % has been achieved via the greedy splitting technique \cite{ZNI05} as well as the divide and conquer technique \cite{OFN12}.

In this work, we will be interested in the submodular $k$-partition problem for subfamilies of submodular functions---namely monotone, symmetric, and posimodular submodular functions. 
A set function $f:2^V\rightarrow \R$ is monotone if $f(A)\le f(B)$ for every $A\subseteq B\subseteq V$, symmetric if $f(A) = f(V-A)$ for every $A\subseteq V$, and posimodular if $f(A)+f(B)\ge f(A- B) + f(B-A)$ for every $A, B\subseteq V$. 
If the input submodular function is monotone/symmetric/posimodular, then we call the associated submodular $k$-partition problem as monotone/symmetric/posimodular submodular $k$-partition. 
 %Two well-known special cases of symmetric submodular $k$-partition problems include graph $k$-cut and hypergraph $k$-partition\footnote{The goal of hypergraph $k$-partition is to compute a partition of the vertex set into $k$ parts that minimizes the sum of the total costs of hyperedges crossing each of the $k$ parts.}---the submodular functions of interest here are the cut functions of an explicitly given graph and hypergraph respectively.
 %A special case of monotone submodular $k$-partition problem is that of matroid $k$-partition---the submodular function of interest here is the matroid rank function. 
 We note that monotone submodular functions and symmetric submodular functions are also posimodular\footnote{In fact, monotone functions are posimodular since $f(A)\ge f(A-B)$ and $f(B)\ge f(B-A)$ for every $A, B\subseteq V$. Symmetric submodular functions are posimodular: for $A, B\subseteq V$, we have that $f(A) + f(B) = f(V-A) + f(B)\ge f((V-A)\cup B) + f((V-A)\cap B)=f(V-(A-B))+f(B-A) =f(A-B)+f(B-A)$.}.  Hence, posimodular submodular $k$-partitioning generalizes both monotone submodular $k$-partitioning and symmetric submodular $k$-partitioning.  
 We now discuss the approximation status of symmetric/monotone/posimodular submodular $k$-partition and some of their well-known special cases  
(see Table \ref{tab: approximation factors} for a summary of approximation factors of symmetric/monotone/posimodular submodular $k$-partition achieved by different approaches).

% A special case of the symmetric submodular $k$-partition problem, the graph $k$-cut problem, is studied using principal partition sequences in \cite{RS07}. In particular, \cite{RS07} gives a $2$-approximation algorithm of graph $k$-cut using principal partition sequences.
%A special case of the symmetric submodular $k$-partition problem is the well-studied graph $k$-cut problem where the submodular function of interest is the cut function of a given graph. 

\paragraph{Symmetric submodular $k$-partition.} 
Graph $k$-cut and hypergraph $k$-partition %\footnote{The goal of hypergraph $k$-partition is to compute a partition of the vertex set into $k$ parts that minimizes the sum of the costs of hyperedges crossing each of the $k$ parts, i.e., minimize $\sum_{i=1}^k (\sum_{e\in \delta(V_i)} c_e)$, where $\delta(V_i)$ is the set of hyperedges that intersect $V_i$ and $V\setminus V_i$.} 
are well-known special cases of symmetric submodular $k$-partition---the submodular functions of interest here are the cut functions of an explicitly given graph and hypergraph respectively.
%Graph $k$-cut is a well-studied special case of symmetric submodular $k$-partition. The submodular function of interest here is the cut function of an explicitly given graph. 
Graph $k$-cut is NP-complete \cite{GH94} and does not have a polynomial-time $(2-\epsilon)$-approximation for every constant $\epsilon>0$ under the Small Set Expansion Hypothesis \cite{Ma18}.
There are several known approaches to achieve a $2$-approximation for graph $k$-cut---(i) 
the greedy splitting approach \cite{SV95}, (ii) the Gomory-Hu tree based approach \cite{Va03}, (iii) the extreme sets based approach \cite{NK07}, (iv) the principal partition sequence based approach \cite{NRP96, Bar00, RS07}, and (v) the covering-LP based approach \cite{NR01, CQX20, Q19}. Greedy splitting, Gomory-Hu tree, and extreme sets based approaches lead to a $(2-2/k)$-approximation while the principal partition sequence and the covering-LP based approaches lead to a $(2-2/n)$-approximation.  
%the greedy splitting approach leads to a $(2-2/k)$-approximation \cite{SV95}, (ii) the Gomory-Hu tree based approach leads to a $(2-2/k)$-approximation \cite{Va03}, (iii) extreme sets based approach leads to a $(2-2/k)$-approximation \cite{NK07}, (iv) the principal partition sequence based approach leads to a $(2-2/n)$-approximation \cite{NRP96, Bar00, RS07}, and (v) a covering-LP based approach leads to a $(2-2/n)$-approximation \cite{NR01, CQX20, Q19}. 
The principal partition sequence and the covering-LP based approaches have also been shown to be related to each other \cite{CQX20}. 
The principal partition sequence based approach is the main algorithm of interest to our work and we will discuss it in detail in Section \ref{sec:pps}.
%The principal partition sequence based algorithm for submodular $k$-partition was introduced by Narayanan, Roy, and Patkar \cite{NRP96} and they also analyzed their algorithm for graph cut functions to show that it achieves a $(2-2/n)$-approximation for graph $k$-cut (which was subsequently rediscovered by Ravi and Sinha \cite{RS07}). %Narayanan, Roy, and Patkar \cite{NRP96} designed an algorithm for the submodular $k$-partition problem based on the principal partition sequence and showed that their algorithm achieves a $(2-2/n)$-approximation for graph $k$-cut (which was subsequently rediscovered by Ravi and Sinha \cite{RS07}). The principal partition sequence based approach is the main algorithm of interest to our work and we will discuss it shortly.
%Saran and Vazirani \cite{SV95} gave a $(2-2/k)$-approximation for graph $k$-cut via greedy splitting. It has also been observed that a $(2-2/k)$-approximation can also be obtained using Gomory-Hu trees \cite{??}. 
%Narayanan, Roy, and Patkar \cite{NRP96} gave a $2$-approximation for graph $k$-cut via the principal partitioning approach which was subsequently rediscovered by Ravi and Sinha \cite{RS07}. 
%\knote{In fact, the principal partition sequence based approach was introduced by Narayanan, Roy, and Patkar who addressed three  generalizations of graph $k$-cut to hypergraphs---can you concisely describe the three variants and the associated approximation factors that they prove?}

For the more general problem of symmetric submodular $k$-partition, two of the  approaches discussed in the previous paragraph for graph $k$-cut have been generalized to obtain $2$-approximations---the greedy splitting approach \cite{ZNI05} and the Gomory-Hu tree approach lead to a $(2-2/k)$-approximation. 
%The motivating goal of our work is 
%Our work was motivated towards 
%understanding the approximationf actor of the principal partition sequence based approach for symmetric submodular $k$-partition.  
Analyzing the approximation factor of the principal partition sequence based approach for symmetric submodular $k$-partition was the starting point of our work. On the inapproximability front, it is known that there does not exist an algorithm that makes polynomial number of function evaluation queries to obtain a $(2-\epsilon)$-approximation for every constant $\epsilon >0$ \cite{San21}. 
%and the Zhao, Nagamochi, and Ibaraki \cite{ZNI05} gave a greedy splitting based approach that achieves a $(2-2/k)$-approximation.
 %The focus of our work is on the fourth approach---namely the principal partition sequence approach. 

 
 \paragraph{Monotone submodular $k$-partition.} 
 Natural cases of monotone submodular $k$-partition problems include matroid $k$-partition and coverage $k$-partition---the submodular function of interest here are matroid rank functions and coverage functions respectively. 
 %It is known that matroid $k$-partition is NP-hard \cite{matroid-k-partition-np-hardness}. 
 It is known that monotone submodular $k$-partition is NP-hard \cite{San21}. 
 Moreover, it admits a simple (and fast) $(2-1/k)$-approximation algorithm that will be denoted henceforth as the \emph{cheapest singleton partitioning algorithm}: return the partition $V_1:=\{v_1\}, V_2:=\{v_2\}, \ldots, V_{k-1}:=\{v_{k-1}\}, V_k:=V-\{v_1, \ldots, v_{k-1}\})$, where the elements are ordered as $v_1, \ldots, v_{n}$ such that $f(\{v_1\})\le f(\{v_2\}) \le \ldots \leq f(\{v_n\})$. Santiago \cite{San21} showed that this is a $2$-approximation. 
 %and it is not difficult to see that it 
 His analysis can be extended to show that it is in fact a $(2-1/k)$-approximation\footnote{The  algorithm returns a solution whose cost is $f(V-V_k)+\sum_{i=1}^{k-1} f(\{v_i\})\le f(V) + \sum_{i=1}^{k-1} f(\{v_i\})\le f(V) + (1-1/k)\sum_{i=1}^{k} f(\{v_i\})\le (2-1/k)\max\{f(V), \sum_{i=1}^k f(\{v_i\})\}$ while the cost of an optimum $k$-partition is at least $\max\{f(V), \sum_{i=1}^k f(\{v_i\})\}$. The lower bound on the cost of the optimum $k$-partition $V_1^*, \ldots, V_k^*$ is because $\sum_{i=1}^k f(V_i^*)\ge f(V)$ by non-negativity and submodularity and moreover, if the optimum partition is indexed such that $\min\{j\in [n]: v_j\in V_i^*\}\le \min\{j\in [n]: v_j\in V_{i+1}^*\}$ for all $i\in [k-1]$, then $f(V_i^*)\ge f(\{v_i\})$ by monotonicity and hence, $\sum_{i=1}^k f(V_i^*)\ge \sum_{i=1}^{k} f(\{v_i\})$. Moreover, $2-1/k$ is the best possible approximation factor for this algorithm: Let $f$ be the rank function of a partition matroid on a $k$-partition $\{S_1,\ldots, S_k\}$ of the ground set $S$ where $|S_i|\geq 2$ for all $i\in[k]$. Then, the algorithm may return $\{\{s_1\}, \{s_2\},\ldots, \{s_{k-1}\}, S-\{s_1, \ldots, s_{k-1}\}\}$, where $s_i\in S_i$ for all $i\in[k-1]$. The returned partition has objective value $2k-1$, whereas the partition $\{S_1,\ldots, S_k\}$ has objective value $k$.}. 
 Alternatively, the greedy splitting algorithm presented in \cite{ZNI05} achieves a $(2-2/k)$-approximation. 
 %a slight modification to the analysis of the greedy splitting algorithm presented in \cite{ZNI05} shows that their algorithm achieves a $(2-2/k)$-approximation for monotone submodular $k$-partition. 
%We note that the greedy splitting algorithm presented in \cite{ZNI05} achieves a $(2-2/k)$-approximation for monotone submodular $k$-partition.
On the inapproximability front, it is known that there does not exist an algorithm that makes polynomial number of function evaluation queries to obtain a $(4/3-\epsilon)$-approximation for every constant $\epsilon>0$ \cite{San21}. 
 
 \paragraph{Posimodular submodular $k$-partition.} The only natural family of posimodular submodular functions that we are familiar with are symmetric submodular functions and monotone submodular functions (as well as their positive linear combinations).
 As mentioned before, posimodular submodular $k$-partition is a unified generalization of symmetric submodular $k$-partition and  monotone submodular $k$-partition.  
 To the best of the authors' knowledge, posimodular submodular $k$-partition has not been studied in the literature before and there are no specialized algorithms or approximation factor analysis of existing algorithms for posimodular submodular $k$-partition.  
 A slight modification to the analysis of the greedy splitting algorithm presented in \cite{ZNI05} shows that their algorithm achieves a $(3-2/k)$-approximation for posimodular submodular $k$-partition---we refrain from presenting this analysis in the interests of brevity. On the inapproximability front, since symmetric submodular functions are also posimodular submodular, it follows that there does not exist an algorithm for posimodular submodular $k$-partition that makes polynomial number of function evaluation queries to obtain a $(2-\epsilon)$-approximation for every constant $\epsilon>0$.   
 %We were able to analyze the  greedy splitting approach of Zhao, Nagamochi, and Ibaraki \cite{ZNI05} to show that it achieves an approximation factor of $3-2/k$ for posimodular submodular $k$-partition.
 %There are no known posimodular submodular $k$-partition problem has no specialized algorithms or analyses so far. The greedy splitting approach of Zhao, Nagamochi, and Ibaraki \cite{ZNI05} achieves an approximation factor of $3-2/k$ for posimodular submodular $k$-partition.
 
 %\paragraph{Principal partition sequence based approach.} 
 %and other special cases of submodular $k$-partition.} 
 %\paragraph{Other special cases of submodular $k$-partition.}

%a greedy splitting based algorithm for submodular $k$-partition that achieves an approximation factor of $2-2/k$ for normalized coverage $k$-partition and hypergraph $k$-partition. On the inapproximability front, hypergraph $k$-cut does not admit an approximation factor of $n^{1/(\log\log n)^c}$, where $c$ is a constant, assuming the Exponential Time Hypothesis \cite{CL20}. 

%\paragraph{Our contributions.} 
\subsection{Our Results}
In this work, we investigate Narayanan, Roy, and Patkar's principal partition sequence based algorithm for submodular $k$-partition \cite{NRP96}. They showed that their algorithm achieves a $(2-2/n)$-approximation for graph $k$-cut (which was subsequently rediscovered by Ravi and Sinha \cite{RS07}).
%Previous works have analyzed their algorithm for graph cut functions and shown that it achieves an approximation factor of $(2-2/n)$ \cite{NRP96, RS07}. 
We show the following results: 
 \begin{enumerate}
 
 \item Their algorithm achieves a $(2-2/n)$-approximation for symmetric submodular $k$-partition. This factor matches the $2$-factor that is known to be achievable by the greedy splitting approach as well as the Gomory-Hu tree approach. Our contribution here is generalizing the analysis of \cite{NRP96, RS07} to beyond graph cut functions. 
 
 \item Their algorithm achieves a $(4/3-4/(9n+3))$-approximation for monotone submodular $k$-partition. This result improves on the trivial $(2-1/k)$-factor that is achieved by the simple singleton partitioning algorithm as well as the $(2-2/k)$-factor that is achieved by the greedy splitting algorithm. Moreover, our upper bound of $4/3$ matches the known lower bound that there does not exist an algorithm that achieves a $(4/3-\epsilon)$-approximation for any constant $\epsilon>0$ using polynomial number of function evaluation queries \cite{San21}. 

 \item Their algorithm achieves a $(2-2/(n+1))$-approximation for posimodular submodular $k$-partition. This result improves on the $3$-factor that is known to be achievable via the greedy splitting technique. 
 
 
 %\item We adapt our analysis of their algorithm for symmetric submodular $k$-partition to show that it achieves a $(2-2/n)$-approximation for monotone submodular $k$-partition and a $(3-3/n)$-approximation for posimodular submodular $k$-partition. 
 %\item The approximation factor of their algorithm is $\Omega(n/k)$ for submodular $k$-partition, where the submodular function can be arbitrary.  
 \end{enumerate}
 \iffalse
 We emphasize that the upper bound on the approximation factor that we show for symmetric submodular $k$-partition is already known to be achievable via the greedy splitting 
 technique: Zhao, Nagamochi, and Ibaraki \cite{ZNI05} showed that their greedy splitting algorithm achieves a  $(2-2/k)$-approximation for symmetric submodular functions. Slight modifications to their analysis show that their algorithm achieves a 
 %approach of Zhao, Nagamochi, and Ibaraki \cite{ZNI05}: it achieves a $(2-2/k)$-approximation for symmetric submodular functions. Their analysis can be adapted to show that it also achieves a 
 $(2-2/k)$-approximation for monotone submodular functions, and a $(3-2/k)$-approximation for posimodular submodular functions. 
 \fi
 See Table \ref{tab: approximation factors} for a comparison. 
 We complement our upper bounds on the approximation factor of their algorithm with matching lower bound constructions.
 Additionally, we show that the approximation factor of their algorithm for arbitrary submodular functions is $\Omega(n/k)$ via a lower bound construction. 
 %We summarize the approximation factor of symmetric/monotone/posimodular submodular $k$-partition achieved by different approaches in Table \ref{tab: approximation factors}.
 %We emphasize that our algorithm of interest that is based on principal partition sequence is identical to the algorithm for submodular $k$-partition designed by Narayanan, Roy, and Patkar  \cite{NRP96} (which was rediscovered and re-analyzed by Ravi and Sinha \cite{RS07} for the special case of graph $k$-cut). Our main contribution is the analysis of its approximation factor for symmetric/monotone/posimodular submodular $k$-partitioning. 
 
% In this work, we show that the principal partition sequence based approach that led to a $(2-2/n)$-approximation for graph $k$-cut also generalizes to lead to a $(2-2/n)$-approximation for \emph{symmetric} submodular $k$-partition. We emphasize that our algorithm based on principal partition sequence is identical to the algorithm of Narayanan, Roy, and Patkar for submodular $k$-partition \cite{NRP96} (which was rediscovered and re-analyzed by Ravi and Sinha \cite{RS07} for the special case of graph $k$-cut). Our main contribution is a tight analysis of its approximation factor for symmetric submodular functions. 
 
% The symmetric submodular $k$-partition problem has a special case \emph{normalized symmetric submodular $k$-partition}. With the same input as symmetric submodular $k$-partition, the goal of normalized symmetric submodular $k$-partition is to compute
% \[\min\left\{\sum_{i\in[k]}f(V_i)-f(V):\{V_1,\ldots, V_k\}\text{ is a partition of }V, V_i\neq\emptyset\;\forall i\in[k]\right\}.\]
% Despite the fact that symmetric submodular $k$-partition and normalized symmetric submodular $k$-partition always have the same optimum value and optimum solution(s), the approximate optima and approximate optimum solution(s) are likely different for these two problems, and thus they are worth independent investigations.

 
%\knote{Do any of the problems considered by NRP address the hypergraph $k$-partition objective---$\sum_{i=1}^k d(V_i)$?}\wnote{I don't think so--the min $k$-overlap problem always comes with the normalizing term.}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    & Graph & Symmetric & Monotone & Posimodular  \\ 
    & Cut Functions & & &\\ 
    \hline
    Greedy splitting& $2-2/k$ \cite{SV95} & $2-2/k$ \cite{ZNI05} & $2-2/k$ \cite{ZNI05} &$3-2/k$ \cite{ZNI05}*\\
    \hline
    Extreme Sets& $2-2/k$ \cite{NK07} &---&---&---\\
    \hline
    Gomory-Hu tree & $2-2/k$ \cite{Va03} & $2-2/k$ [Folklore] & --- & --- \\
    \hline
    Covering-LP &$2-2/k$ \cite{NR01, CQX20}&---&---&---\\
    \hline
    Cheapest Singleton &---&---&$2-1/k$ [Folklore]&---\\
     Partitioning & & & & \\
     \hline
    Principle Partition & $2-2/n$ \cite{NRP96, RS07} & $2-2/n$  & $4/3-4/(9n+3)$ & $2-2/(n+1)$ \\
    Sequence & & & &\\
    \hline
    \textbf{Lower Bound} & \textbf{$2-\epsilon$} \cite{Ma18} & $2-\epsilon$ \cite{San21}& $4/3-\epsilon$ \cite{San21} & $2-\epsilon$ \cite{San21}\\
    \hline
    \end{tabular}
    \caption{Approximation factors of symmetric/monotone/posimodular submodular $k$-partition using difference approaches. Graph $k$-cut is the well-studied special case of symmetric submodular $k$-partition, so we include that as the first column for comparison. 
    Result marked with an asterisk follow by slight modifications to the known analysis of the approximation factor for symmetric submodular functions given in \cite{ZNI05}. Approximation factors in the row corresponding to principle partition sequence are the main results of this work. In the last row, we include the known lower bounds on the approximation factor for comparison. The lower bound for graph cut functions is assuming the small set expansion hypothesis while the rest of the lower bounds are assuming polynomial number of function evaluation queries.}
    \label{tab: approximation factors}
\end{table}


\paragraph{Organization.} We discuss the principal partition sequence based algorithm in detail in Section \ref{sec:pps}. We analyze the approximation factor of the algorithm with matching lower bound constructions for each of the three subfamilies of submodular functions in Section \ref{sec:approx-analysis}. We exhibit an instance of submodular $k$-partition where the algorithm achieves an approximation factor of $\Omega(n/k)$ in Section \ref{subsec: PPS n/k-apx}.  


 \subsection{Related work} 
 The principal partition sequence based approach for submodular $k$-partition was introduced by Narayanan, Roy, and Patkar \cite{NRP96}. We will formally discuss their algorithm in Section \ref{sec:pps}. They analyzed the approximation factor of their algorithm for two variants of $k$-partitioning problems in hypergraphs. 
%shown by the same authors to two generalizations of the graph $k$-cut problem to hypergraphs.
%---the min-$k$-vertex sharing problem and the min-$k$-overlap problem. In particular, the min-$k$-vertex sharing problem addresses two hypergraph $k$-partition problems.
 These two variants are not special cases of symmetric/monotone/posimodular submodular $k$-partition and are not of direct interest to our work. However, we describe them in the interests of %for the sake of completeness. 
 presenting a complete picture on the applicability of the principal partition sequence based approach. 
Given a hypergraph $H=(V,E)$, a hyperedge cost function $c:E\to\R_+$, and an integer $k$, the goal is to find a partition $\mcp:=\{V_1,\ldots,V_k\}$ of $V$ that minimizes an objective of interest: 
\begin{enumerate}
    \item If the objective is the total cost of hyperedges that intersect at least two parts of $\mcp$, then the problem is known as \emph{hypergraph $k$-cut}. 
    \item If the objective is the sum of cost of hyperedges relative to the partition $\mcp$, where the cost of a hyperedge $e$ relative to $\mcp$ is $c(e)(\ell-1)$ with $\ell$ being the number of parts of $\mcp$ intersected by $e$, then the problem is known as \emph{normalized coverage $k$-partition}\footnote{The nomenclature is because the problem is equivalent to finding a partition $V_1, \ldots, V_k$ of the ground set $V$ so as to minimize $\sum_{i=1}^k f(V_i) - f(V)$, where $f:2^V\rightarrow \R_+$ is an explicitly given coverage function (every coverage function can be uniquely represented using a hypergraph \cite{CH12}). Here, subtracting $f(V)$ gives a stronger objective for the purpose of approximation since it is a trivial lower bound on the sum of the function values of the parts: $\sum_{i=1}^k f(V_i)\ge f(V)$ holds for every $k$-partition $V_1, \ldots, V_k$.}.  
    %The total cost of hyperedges that intersect at least two parts of $\mcp$, where each hyperedge cost is counted $\ell-1$ times if it intersects exactly $\ell$ parts of $\mcp$. 
    %\knote{We will call the associated problem as \emph{normalized coverage $k$-partition} since it is equivalent to finding a partition $V_1, \ldots, V_k$ of the ground set $V$ so as to minimize $\sum_{i=1}^k f(V_i) - f(V)$, where $f:2^V\rightarrow \R_+$ is an explicitly given coverage function\footnote{A  function $f:2^V \rightarrow \R_+$ is a coverage function if there exist a finite set $[m]$ along with weights $w:[m]\rightarrow \R_+$ and sets $S_v$ for each $v\in V$ such that $f(A)=\sum_{e\in \cup_{v\in A}S_v}w(e)$. Every coverage function can be uniquely represented using a hypergraph \cite{CH12}.}. Here, subtracting $f(V)$ is reasonable since it is a trivial lower bound on the sum of the function values of the parts: $\sum_{i=1}^k f(V_i)\ge f(V)$ holds for every $k$-partition $V_1, \ldots, V_k$.}
\end{enumerate}
%We note that both these variants are special cases of submodular $k$-partition but are not special cases of symmetric submodular $k$-partition.  
%(in contrast to hypergraph $k$-partition which is indeed a special case of symmetric submodular $k$-partition). 
Narayanan, Roy, and Patkar \cite{NRP96} used the principal partition sequence approach to design a $r(1-1/n)$-approximation for hypergraph $k$-cut where $r$ is the size of the largest hyperedge in $H$ and a $(2-2/n)$-approximation for normalized coverage $k$-partition.
% \wnote{In page 318 of NPR96, the approximation factor is stated as $r(1-1/n)$} 
As a consequence, their algorithm implies a $(2-2/n)$-approximation for graph $k$-cut (since $r=2$). 

We mention that a slight modification to the analysis of the greedy splitting algorithm presented in \cite{ZNI05} shows that their algorithm achieves a $(2-2/k)$-approximation for normalized coverage $k$-partition and hypergraph $k$-partition. 
%We mention that we were able to adapt the analysis of the greedy splitting based algorithm for submodular $k$-partition designed by Zhao, Nagamochi, and Ibaraki \cite{ZNI05} to conclude that their algorithm achieves a $(2-2/k)$-approximation for normalized coverage $k$-partition and hypergraph $k$-partition, but we don't present these analysis since they are not the central results of this work. 
On the inapproximability front, it is known that hypergraph $k$-cut does not admit an approximation factor of $n^{1/(\log\log n)^c}$, where $c$ is a constant, assuming the Exponential Time Hypothesis \cite{CL20}. The strongest-known inapproximability result for the more general submodular $k$-partition problem follows from this inapproximability for hypergraph $k$-cut. 



==> intro-old.tex <==
\section{Introduction}\label{sec:intro}
A set function $f:2^V\rightarrow \R$ is submodular if $f(A)+f(B)\ge f(A\cap B) + f(A\cup B)$ for every $A, B\subseteq V$. 
We consider the \emph{submodular $k$-partition} problem defined as follows: The input consists of a non-negative submodular function $f:2^V\to\R_{\geq 0}$ on ground set $V$ of size $n$ via an evaluation oracle and an integer $k\geq 2$. The goal is to find a partition $V_1,\ldots,V_k$ of $V$ into $k$ non-empty parts in order to minimize $\sum_{i=1}^k f(V_i)$. Namely, the goal is to compute
\[\min\left\{\sum_{i\in[k]}f(V_i):\{V_1,\ldots, V_k\}\text{ is a partition of }V,\ V_i\neq\emptyset\;\forall i\in[k]\right\}.\]
The set function $f:2^V\rightarrow \R$ is symmetric if $f(A) = f(V-A)$ for every $A\subseteq V$, monotone if $f(A)\le f(B)$ for every $A\subseteq B\subseteq V$, and posimodular if $f(A)+f(B)\ge f(A- B) + f(B-A)$ for every $A, B\subseteq V$. 
If the input function is symmetric/monotone/posimodular, then we call the problem as \emph{symmetric/monotone/posimodular} submodular $k$-partition.
 Two well-known special cases of symmetric submodular $k$-partition problems include graph $k$-cut and hypergraph $k$-partition---the submodular functions of interest here are the cut functions of an explicitly given graph and hypergraph respectively. 
 A special case of monotone submodular $k$-partition problem is that of matroid $k$-partition---the submodular function of interest here is the matroid rank function. We note that monotone submodular functions and symmetric submodular functions are also posimodular. Hence, posimodular submodular $k$-partitioning generalizes both symmetric submodular $k$-partitioning and monotone submodular $k$-partitioning.  

 \knote{Might be better to refer to NRP's principal partition sequence based algorithm for submodular $k$-partitioning already at this point and state the results?}


% A special case of the symmetric submodular $k$-partition problem, the graph $k$-cut problem, is studied using principal partition sequences in \cite{RS07}. In particular, \cite{RS07} gives a $2$-approximation algorithm of graph $k$-cut using principal partition sequences.
%A special case of the symmetric submodular $k$-partition problem is the well-studied graph $k$-cut problem where the submodular function of interest is the cut function of a given graph. 

Graph $k$-cut is a well-studied special case of symmetric submodular $k$-partition. It 
%Graph $k$-cut 
is NP-complete \cite{GH88} and does not have a polynomial-time $(2-\epsilon)$-approximation for every constant $\epsilon>0$ under the Small Set Expansion Hypothesis \cite{Ma18}.
There are several known approaches to achieve a $2$-approximation for graph $k$-cut---(i) the greedy splitting approach leads to a $(2-2/k)$-approximation \cite{SV95}, (ii) the Gomory-Hu tree based approach leads to a $(2-2/k)$-approximation \cite{Va03}, (iii) extreme sets based approach leads to a $(2-2/k)$-approximation \cite{NK07}, (iv) the principal partition sequence based approach leads to a $(2-2/n)$-approximation \cite{NRP96, Bar00, RS07}, and (v) a covering-LP based approach leads to a $(2-2/n)$-approximation \cite{NR01, CQX20, Q19}. The covering-LP and the principal partition sequence based approach have also been shown to be related to each other \cite{CQX20}.   
%Saran and Vazirani \cite{SV95} gave a $(2-2/k)$-approximation for graph $k$-cut via greedy splitting. It has also been observed that a $(2-2/k)$-approximation can also be obtained using Gomory-Hu trees \cite{??}. 
%Narayanan, Roy, and Patkar \cite{NRP96} gave a $2$-approximation for graph $k$-cut via the principal partitioning approach which was subsequently rediscovered by Ravi and Sinha \cite{RS07}. 
%\knote{In fact, the principal partition sequence based approach was introduced by Narayanan, Roy, and Patkar who addressed three  generalizations of graph $k$-cut to hypergraphs---can you concisely describe the three variants and the associated approximation factors that they prove?}

For the more general problem of symmetric submodular $k$-partition, two of the  approaches discussed in the previous paragraph for graph $k$-cut have been generalized to obtain $2$-approximations---the greedy splitting approach \cite{ZNI05} and the Gomory-Hu tree approach lead to $(2-2/k)$-approximations. 
 %and the Zhao, Nagamochi, and Ibaraki \cite{ZNI05} gave a greedy splitting based approach that achieves a $(2-2/k)$-approximation.
 The focus of our work is on the fourth approach---namely the principal partition sequence approach. Narayanan, Roy, and Patkar \cite{NRP96} designed an algorithm for the submodular $k$-partition problem based on the principal partition sequence and showed that their algorithm achieves a $(2-2/n)$-approximation for graph $k$-cut (which was subsequently rediscovered by Ravi and Sinha \cite{RS07}). In this work, we investigate Narayanan, Roy, and Patkar's principal partition sequence based algorithm and show the following results:
 \begin{enumerate}
 \item Their algorithm achieves a $(2-2/n)$-approximation for symmetric submodular $k$-partition.
 \item We adapt our analysis of their algorithm for symmetric submodular $k$-partition to show that it achieves a $(2-2/n)$-approximation for monotone submodular $k$-partition and a $(3-3/n)$-approximation for posimodular submodular $k$-partition. 
 \item The approximation factor of their algorithm is $\Omega(n/k)$ for submodular $k$-partition, where the submodular function can be arbitrary.  
 \end{enumerate}
 We emphasize that the upper bound on the approximation factors that we show are already known to be achievable via the greedy splitting approach of Zhao, Nagamochi, and Ibaraki \cite{ZNI05}: it achieves a $(2-2/k)$-approximation for symmetric submodular functions, a $(2-2/k)$-approximation for monotone submodular functions, and a $(3-2/k)$-approximation for posimodular submodular functions. Our main contribution here is analyzing the approximation factor of the principal partition sequence approach.
 %We emphasize that our algorithm of interest that is based on principal partition sequence is identical to the algorithm for submodular $k$-partition designed by Narayanan, Roy, and Patkar  \cite{NRP96} (which was rediscovered and re-analyzed by Ravi and Sinha \cite{RS07} for the special case of graph $k$-cut). Our main contribution is the analysis of its approximation factor for symmetric/monotone/posimodular submodular $k$-partitioning. 
 
% In this work, we show that the principal partition sequence based approach that led to a $(2-2/n)$-approximation for graph $k$-cut also generalizes to lead to a $(2-2/n)$-approximation for \emph{symmetric} submodular $k$-partition. We emphasize that our algorithm based on principal partition sequence is identical to the algorithm of Narayanan, Roy, and Patkar for submodular $k$-partition \cite{NRP96} (which was rediscovered and re-analyzed by Ravi and Sinha \cite{RS07} for the special case of graph $k$-cut). Our main contribution is a tight analysis of its approximation factor for symmetric submodular functions. 
 
% The symmetric submodular $k$-partition problem has a special case \emph{normalized symmetric submodular $k$-partition}. With the same input as symmetric submodular $k$-partition, the goal of normalized symmetric submodular $k$-partition is to compute
% \[\min\left\{\sum_{i\in[k]}f(V_i)-f(V):\{V_1,\ldots, V_k\}\text{ is a partition of }V, V_i\neq\emptyset\;\forall i\in[k]\right\}.\]
% Despite the fact that symmetric submodular $k$-partition and normalized symmetric submodular $k$-partition always have the same optimum value and optimum solution(s), the approximate optima and approximate optimum solution(s) are likely different for these two problems, and thus they are worth independent investigations.

\paragraph{Related work.} 
We refer the reader to \cite{CC22-j} for a discussion on the status of submodular $k$-partition problem for fixed constant $k$. The focus of this work is on submodular $k$-partitioning problem where $k$ is part of input. For arbitrary submodular functions (not necessarily symmetric), the best-known approximation factor is $O(k)$ and it can be achieved via the greedy splitting technique \cite{ZNI05} and the divide and conquer technique \cite{OFN12}. For monotone submodular functions, there is a simple $2$-approximation algorithm: return the partition $V_1:=\{v_1\}, V_2:=\{v_2\}, \ldots, V_{k-1}:=\{v_{k-1}\}, V_k:=V-\{v_1, \ldots, v_{k-1}\})$, where the elements are ordered as $v_1, \ldots, v_{n}$ such that $f(\{v_1\})\le f(\{v_2\}) \le \ldots \leq f(\{v_n\})$\footnote{The optimum value is at least $\max\{f(V), \sum_{i=1}^k f(\{v_i\})\}$ while the algorithm returns a solution whose cost is $f(V-V_k)+\sum_{i=1}^{k-1} f(\{v_i\})\le f(V) + \sum_{i=1}^{k-1} f(\{v_i\})\le f(V) + (1-1/k)\sum_{i=1}^{k} f(\{v_i\})\le (2-1/k)\max\{f(V), \sum_{i=1}^k f(\{v_i\})\}$. The lower bound on the cost of the optimum $k$-partition $V_1^*, \ldots, V_k^*$ is because $\sum_{i=1}^k f(V_i^*)\ge f(V)$ by non-negativity and submodularity and moreover, if the optimum partition is indexed such that $\min\{j\in [n]: v_j\in V_i^*\}\le \min\{j\in [n]: v_j\in V_{i+1}^*\}$, then $f(V_i^*)\ge f(\{v_i\})$ by monotonicity and hence, $\sum_{i=1}^k f(V_i^*)\ge \sum_{i=1}^{k} f(\{v_i\})$.}. 
We note that the greedy splitting technique also leads to a $(2-2/k)$-approximation for monotone submodular functions \cite{ZNI05}.\knote{Is there a  $(2-\epsilon)$-inapproximability for monotone submodular $k$-partition? E.g., $k$-partition for matroid rank functions? See if ZNI say something about the tightness of their Greedy Splitting Algorithm for monotone submodular $k$-partition.}

The principal partition sequence based approach for submodular $k$-partition was introduced by Narayanan, Roy, and Patkar \cite{NRP96}. They analyzed the approximation factor of the approach for two variants of $k$-partitioning problems in hypergraphs. 
%shown by the same authors to two generalizations of the graph $k$-cut problem to hypergraphs.
%---the min-$k$-vertex sharing problem and the min-$k$-overlap problem. In particular, the min-$k$-vertex sharing problem addresses two hypergraph $k$-partition problems.
 Although these two variants are not special cases of symmetric/monotone/posimodular submodular $k$-partition, we describe them for the sake of completeness. 
Given a hypergraph $H=(V,E)$, a hyperedge cost function $c:E\to\R_+$, and an integer $k$, the goal is to find a partition $\mcp:=\{V_1,\ldots,V_k\}$ of $V$ that minimizes an objective of interest: 
\begin{enumerate}
    \item If the objective is the total cost of hyperedges that intersect at least two parts of $\mcp$, then the problem is known as \emph{hypergraph $k$-cut}. 
    \item If the objective is the sum of cost of hyperedges relative to the partition $\mcp$, where the cost of a hyperedge $e$ relative to $\mcp$ is $c(e)(\ell-1)$, where $\ell$ is the number of parts of $\mcp$ intersected by $e$, then the problem is known as \emph{normalized coverage $k$-partition}\footnote{The nomenclature is because the problem is equivalent to finding a partition $V_1, \ldots, V_k$ of the ground set $V$ so as to minimize $\sum_{i=1}^k f(V_i) - f(V)$, where $f:2^V\rightarrow \R_+$ is an explicitly given coverage function (every coverage function can be uniquely represented using a hypergraph \cite{CH12}). Here, subtracting $f(V)$ gives a stronger objective for the purpose of approximation since it is a trivial lower bound on the sum of the function values of the parts: $\sum_{i=1}^k f(V_i)\ge f(V)$ holds for every $k$-partition $V_1, \ldots, V_k$.}.  
    %The total cost of hyperedges that intersect at least two parts of $\mcp$, where each hyperedge cost is counted $\ell-1$ times if it intersects exactly $\ell$ parts of $\mcp$. 
    %\knote{We will call the associated problem as \emph{normalized coverage $k$-partition} since it is equivalent to finding a partition $V_1, \ldots, V_k$ of the ground set $V$ so as to minimize $\sum_{i=1}^k f(V_i) - f(V)$, where $f:2^V\rightarrow \R_+$ is an explicitly given coverage function\footnote{A  function $f:2^V \rightarrow \R_+$ is a coverage function if there exist a finite set $[m]$ along with weights $w:[m]\rightarrow \R_+$ and sets $S_v$ for each $v\in V$ such that $f(A)=\sum_{e\in \cup_{v\in A}S_v}w(e)$. Every coverage function can be uniquely represented using a hypergraph \cite{CH12}.}. Here, subtracting $f(V)$ is reasonable since it is a trivial lower bound on the sum of the function values of the parts: $\sum_{i=1}^k f(V_i)\ge f(V)$ holds for every $k$-partition $V_1, \ldots, V_k$.}
\end{enumerate}
We note that both these variants are special cases of submodular $k$-partition but are not special cases of symmetric submodular $k$-partition (in contrast to hypergraph $k$-partition which is indeed a special case of symmetric submodular $k$-partition). 
Narayanan, Roy, and Patkar \cite{NRP96} used the principal partition sequence approach to design a $(2-2/n)$-approximation for normalized coverage $k$-partition, and a $r(1-1/n)$-approximation for hypergraph $k$-cut, where $r$ is the size of the largest hyperedge in $H$.
% \wnote{In page 318 of NPR96, the approximation factor is stated as $r(1-1/n)$} 
As a consequence, their algorithm implies a $(2-2/n)$-approximation for graph $k$-cut (since $r=2$). 

Zhao, Nagamochi, and Ibaraki \cite{ZNI05} designed a greedy splitting based algorithm for submodular $k$-partition that achieves an approximation factor of $2-2/k$ for normalized coverage $k$-partition and hypergraph $k$-partition. On the inapproximability front, hypergraph $k$-cut does not admit an approximation factor of $n^{1/(\log\log n)^c}$, where $c$ is a constant, assuming the Exponential Time Hypothesis \cite{CL20}. 
%\knote{Do any of the problems considered by NRP address the hypergraph $k$-partition objective---$\sum_{i=1}^k d(V_i)$?}\wnote{I don't think so--the min $k$-overlap problem always comes with the normalizing term.}

\paragraph{Organization.} \knote{TODO.}


==> monotone-1.tex <==
\subsection{Monotone submodular functions}\label{sec:mono}
We adapt our analysis of the approximation factor of Algorithm 1 for symmetric submodular $k$-partitioning to monotone submodular $k$-partitioning in this section to prove the following theorem. 

\begin{theorem} \label{Thm: 2-approx mono sm k-cut algo}
The approximation factor of Algorithm 1 for non-negative monotone  submodular $k$-partitioning is $2(1-1/n)$, where $n$ is the size of the ground set. 
\end{theorem}


We present the analysis of the approximation factor of Algorithm 1 for non-negative monotone submodular functions only to illustrate the generality of Algorithm 1 and emphasize that there is a much simpler $2$-approximation for non-negative monotone submodular functions (see Section \ref{sec:intro}). 
Lemmas \ref{claim:exact-k} and \ref{lemma:monotone} complete the proof of Theorem \ref{Thm: 2-approx mono sm k-cut algo}. 

\begin{lemma}\label{lemma:monotone}
Let $k\geq 2$ be an integer, $f:2^V\to\R_{\ge 0}$ be a non-negative monotone submodular function on a ground set $V$ of size $n$, $\mcp^\ast$ be a $k$-partition of $V$ that minimizes $f(\mcp^\ast)$, and $\mcp_1, \mcp_2, \ldots, \mcp_r$ be the principal partition sequence of the submodular function $f$ satisfying the conditions of Theorem \ref{Thm: PPS}. 
Suppose $|\mcp_j|\neq k$ for all $j\in[r]$.
%Let $\mcp_{i-1},\mcp_i$ be the partitions such that $|\mcp_{i-1}|<k<|\mcp_i|$. 
%If $|\mcp_j|\neq k$ for all $j\in[r]$, 
Then, the partition $\mcp$ returned by Algorithm 1
%\ref{Algo: 2-approx sym sm k-partition} 
satisfies 
\[f(\mcp)\leq 2\left(1-\frac{1}{n}\right)f(\mcp^\ast).\]
\iffalse
Suppose $f:2^V\rightarrow \R_{\ge 0}$ is monotone. If $|\mcp_j|\neq k$ for all $j\in[r]$, then the partition $\mcp$ returned by Algorithm 1 satisfies 
\[f(\mcp)\leq 2\left(1-\frac{1}{n}\right)f(\mcp^\ast).\]
\fi
\end{lemma}

\begin{proof}
Let $\mcp_{i-1},\mcp_i$ be the partitions in Algorithm 1 such that $|\mcp_{i-1}|<k<|\mcp_i|$. Let $S$ and $\mcp'=\{B_1,B_2,\ldots,B_{|\mcp'|}\}$ be as in Algorithm 1. 

Firstly, since $\cup_{j=k-|\mcp_{i-1}|+1}^{|\mcp'|} B_j \subseteq S$ and $f$ is monotone, we have that 
\[
f\left(\cup_{j=k-|\mcp_{i-1}|+1}^{|\mcp'|} B_j\right) \le f(S).
\]
Secondly, by our choice of $B_1,B_2,\ldots,B_{k-|\mcp_{i-1}|}$, we know that
\begin{align}
    \sum_{j=1}^{k-|\mcp_{i-1}|}f(B_j)\leq\frac{k-|\mcp_{i-1}|}{|\mcp'|}f(\mcp').\label{Eqn: sum of f(Bj) second}
\end{align}
Hence,
\begin{align*}
    f(\mcp)&=f(\mcp_{i-1})-f(S)+\sum_{j=1}^{k-|\mcp_{i-1}|}f(B_j)+f\left(\bigcup_{j=k-|\mcp_{i-1}|+1}^{|\mcp'|}B_j\right)
    \\&\leq f(\mcp_{i-1})+\sum_{j=1}^{k-|\mcp_{i-1}|}f(B_j)
    \\&\leq f(\mcp_{i-1})+\frac{k-|\mcp_{i-1}|}{|\mcp'|}f(\mcp')
    \\&=f(\mcp_{i-1})+\frac{k-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}(f(\mcp_i)+f(S)-f(\mcp_{i-1})),
\end{align*}
where the last equality follows from the fact that $f(\mcp_{i-1})-f(S)+f(\mcp')=f(\mcp_i)$ and $|\mcp'|=|\mcp_i|-|\mcp_{i-1}|+1$. Rearranging, we have
% \begin{align*}
%     f(\mcp)&\leq \frac{f(\mcp_{i-1})}{|\mcp_i|-|\mcp_{i-1}|+1}(|\mcp_i|-k+1)+\frac{f(\mcp_{i})}{|\mcp_i|-|\mcp_{i-1}|+1}(k-|\mcp_{i-1}|)+\frac{f(S)}{|\mcp_i|-|\mcp_{i-1}|+1}(k-|\mcp_{i-1}|)
%     \\&=\left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\left(\frac{f(\mcp_{i-1})}{|\mcp_i|-|\mcp_{i-1}|}(|\mcp_i|-k+1)+\frac{f(\mcp_{i})+f(S)}{|\mcp_i|-|\mcp_{i-1}|}(k-|\mcp_{i-1}|)\right)
%     \\&\le\left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\left(\frac{f(\mcp_{i-1})}{|\mcp_i|-|\mcp_{i-1}|}(2|\mcp_i|-2k)+\frac{f(\mcp_{i})+f(S)}{|\mcp_i|-|\mcp_{i-1}|}(k-|\mcp_{i-1}|)\right) \quad(\text{since $1\le |\mcp_i|-k$})
%     \\&\le\left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\left(\frac{f(\mcp_{i-1})}{|\mcp_i|-|\mcp_{i-1}|}(2|\mcp_i|-2k)+\frac{2f(\mcp_{i})}{|\mcp_i|-|\mcp_{i-1}|}(k-|\mcp_{i-1}|)\right) \quad(\text{since }f(S)\leq f(\mcp_i))
%     \\&\leq \left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\cdot 2f(\mcp^\ast)\quad(\text{by Claim \ref{lemma: f long ineq}})
%     \\&= \left(1-\frac{1}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\cdot 2f(\mcp^\ast)
%     \\&\leq 2\left(1-\frac{1}{n}\right)f(\mcp^\ast),
% \end{align*}
\begin{align*}
    f(\mcp)&\leq \frac{f(\mcp_{i-1})}{|\mcp_i|-|\mcp_{i-1}|+1}(|\mcp_i|-k+1)+\frac{f(\mcp_{i})}{|\mcp_i|-|\mcp_{i-1}|+1}(k-|\mcp_{i-1}|)+\frac{f(S)}{|\mcp_i|-|\mcp_{i-1}|+1}(k-|\mcp_{i-1}|)
    \\&=\left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\left(\frac{f(\mcp_{i-1})}{|\mcp_i|-|\mcp_{i-1}|}(|\mcp_i|-k+1)+\frac{f(\mcp_{i})+f(S)}{|\mcp_i|-|\mcp_{i-1}|}(k-|\mcp_{i-1}|)\right)
    \\&\leq \left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\left(f(\mcp^\ast) + \frac{f(\mcp_{i-1})}{|\mcp_i|-|\mcp_{i-1}|} +\frac{f(S)}{|\mcp_i|-|\mcp_{i-1}|}(k-|\mcp_{i-1}|)\right) \quad(\text{by Lemma \ref{lemma: f long ineq}})
    \\&\leq \left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\left(f(\mcp^\ast) +\frac{f(\mcp_{i-1})}{|\mcp_i|-|\mcp_{i-1}|}(1+k-|\mcp_{i-1}|)\right)  \quad(\text{since $f(S)\leq f(\mcp_{i-1})$})
    \\&\leq \left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\left(f(\mcp^\ast) +f(\mcp_{i-1})\right) \quad(\text{since $|\mcp_i|\ge 1+k$})
    \\&\leq \left(\frac{|\mcp_i|-|\mcp_{i-1}|}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\cdot 2f(\mcp^\ast)\quad(\text{by Lemma \ref{lemma: f long ineq}})
    \\&= \left(1-\frac{1}{|\mcp_i|-|\mcp_{i-1}|+1}\right)\cdot 2f(\mcp^\ast)
    \\&\leq 2\left(1-\frac{1}{n}\right)f(\mcp^\ast),
\end{align*}
where the last inequality is because $|\mcp_i|-|\mcp_{i-1}|\leq n-1$. 
%We note that Claim \ref{lemma: f long ineq} does not assume symmetry of $f$, and thus remains applicable.
\end{proof}

\knote{Tight example?} \wnote{There exists an example with $n=3$ and the algorithm returns a $6/5$-approximation.}

